Perturbations of Dark Solitons

A method for approximating dark soliton solutions of the nonlinear Schrodinger equation under the influence of perturbations is presented. The problem is broken into an inner region, where core of the soliton resides, and an outer region, which evolves independently of the soliton. It is shown that a shelf develops around the soliton which propagates with speed determined by the background intensity. Integral relations obtained from the conservation laws of the nonlinear Schrodinger equation are used to approximate the shape of the shelf. The analysis is developed for both constant and slowly evolving backgrounds. A number of problems are investigated including linear and nonlinear damping type perturbations.

==> MainBib.tex <==
@article{ Karpman1977,
Author = {KARPMAN, VI and MASLOV, EM},
Title = {{Perturbation-Theroy for Solitons}},
Journal = {{ZHURNAL EKSPERIMENTALNOI I TEORETICHESKOI FIZIKI}},
Year = {{1977}},
Volume = {{73}},
Number = {{2}},
Pages = {{537-559}},
ISSN = {{0044-4510}},
Unique-ID = {{ISI:A1977DS53600020}},
}


@article{ Kodama1981,
Author = {KODAMA, Y and ABLOWITZ, MJ},
Title = {{Perturbations of Solitons and Solitary Waves}},
Journal = {{STUDIES IN APPLIED MATHEMATICS}},
Year = {{1981}},
Volume = {{64}},
Number = {{3}},
Pages = {{225-245}},
ISSN = {{0022-2526}},
Unique-ID = {{ISI:A1981LU51900003}},
}


@article{ HermanRL1990,
Author = {HERMAN, RL},
Title = {{A Direct Approach to Studying Soliton Perturbations}},
Journal = {{JOURNAL OF PHYSICS A-MATHEMATICAL AND GENERAL}},
Year = {{1990}},
Volume = {{23}},
Number = {{12}},
Pages = {{2327-2362}},
Month = {{JUN 21}},
ISSN = {{0305-4470}},
Unique-ID = {{ISI:A1990DK46100017}},
}


@article{ Emplit1987,
Author = {EMPLIT, P and HAMAIDE, JP and REYNAUD, F and FROEHLY, C and BARTHELEMY,
   A},
Title = {{Picosecond Steps and Dark Pulses Through Nonlinear Single-Mode Fibers}},
Journal = {{OPTICS COMMUNICATIONS}},
Year = {{1987}},
Volume = {{62}},
Number = {{6}},
Pages = {{374-379}},
Month = {{JUN 15}},
ISSN = {{0030-4018}},
Unique-ID = {{ISI:A1987J207000003}},
}


@article{ Andersen1991,
Author = {SWARTZLANDER, GA and ANDERSEN, DR and REGAN, JJ and YIN, H and KAPLAN,
   AE},
Title = {{Spatial Dark-Soliton Stripes and Grids in Self-Defocusing Materials}},
Journal = {{PHYSICAL REVIEW LETTERS}},
Year = {{1991}},
Volume = {{66}},
Number = {{12}},
Pages = {{1583-1586}},
Month = {{MAR 25}},
ISSN = {{0031-9007}},
Unique-ID = {{ISI:A1991FC78000010}},
}


@article{ Zhao1989,
Author = {ZHAO, W and BOURKOFF, E},
Title = {{Propagation Properties of Dark Solitons}},
Journal = {{OPTICS LETTERS}},
Year = {{1989}},
Volume = {{14}},
Number = {{13}},
Pages = {{703-705}},
Month = {{JUL 1}},
ISSN = {{0146-9592}},
Unique-ID = {{ISI:A1989AC82100017}},
}


@article{ Giannini1990,
Author = {GIANNINI, JA and JOSEPH, RI},
Title = {{The Propagation of Bright and Dark Solitons in Lossy Optical Fibers}},
Journal = {{IEEE JOURNAL OF QUANTUM ELECTRONICS}},
Year = {{1990}},
Volume = {{26}},
Number = {{12}},
Pages = {{2109-2114}},
Month = {{DEC}},
ISSN = {{0018-9197}},
Unique-ID = {{ISI:A1990EY43900011}},
}


@article{ Lisak1991,
Author = {LISAK, M and ANDERSON, D and MALOMED, BA},
Title = {{Dissipative Damping of Dark Solitons in Optical Fibers}},
Journal = {{OPTICS LETTERS}},
Year = {{1991}},
Volume = {{16}},
Number = {{24}},
Pages = {{1936-1937}},
Month = {{DEC 15}},
ISSN = {{0146-9592}},
Unique-ID = {{ISI:A1991GY73100008}},
}


@article{ Kivshar1994,
Author = {KIVSHAR, YS and YANG, XP},
Title = {{Perturbation-Induced Dynamics of Dark Solitons}},
Journal = {{PHYSICAL REVIEW E}},
Year = {{1994}},
Volume = {{49}},
Number = {{2}},
Pages = {{1657-1670}},
Month = {{FEB}},
ISSN = {{1063-651X}},
Unique-ID = {{ISI:A1994NA92100091}},
}


@article{ Konotop1994,
Author = {KONOTOP, VV and VEKSLERCHIK, VE},
Title = {{Direct Perturbation-Theroy for Dark Solitons}},
Journal = {{PHYSICAL REVIEW E}},
Year = {{1994}},
Volume = {{49}},
Number = {{3}},
Pages = {{2397-2407}},
Month = {{MAR}},
ISSN = {{1063-651X}},
Unique-ID = {{ISI:A1994NC46500074}},
}


@article{ Kaup1976,
Author = {KAUP, DJ},
Title = {{Perturbation Expansion for Zakharov-Shabat Inverse Scattering Transform}},
Journal = {{SIAM JOURNAL ON APPLIED MATHEMATICS}},
Year = {{1976}},
Volume = {{31}},
Number = {{1}},
Pages = {{121-133}},
ISSN = {{0036-1399}},
Unique-ID = {{ISI:A1976BW23000013}},
}


@article{ Ao2005,
Author = {Ao, SM and Yan, JR},
Title = {{A perturbation method for dark solitons based on a complete set of the
   squared Jost solutions}},
Journal = {{JOURNAL OF PHYSICS A-MATHEMATICAL AND GENERAL}},
Year = {{2005}},
Volume = {{38}},
Number = {{11}},
Pages = {{2399-2413}},
Month = {{MAR 18}},
DOI = {{10.1088/0305-4470/38/11/006}},
ISSN = {{0305-4470}},
Unique-ID = {{ISI:000228576200007}},
}


@article{ Chen1998,
Author = {Chen, XJ and Chen, ZD and Huang, NN},
Title = {{Completeness of squared Jost solutions for dark solitons}},
Journal = {{PROGRESS IN NATURAL SCIENCE}},
Year = {{1998}},
Volume = {{8}},
Number = {{6}},
Pages = {{672-678}},
Month = {{DEC}},
ISSN = {{1002-0071}},
Unique-ID = {{ISI:000078714100004}},
}


@article{ Lashkin2004,
Author = {Lashkin, VM},
Title = {{Perturbation theory for dark solitons: Inverse scattering transform
   approach and radiative effects}},
Journal = {{PHYSICAL REVIEW E}},
Year = {{2004}},
Volume = {{70}},
Number = {{6, Part 2}},
Month = {{DEC}},
DOI = {{10.1103/PhysRevE.70.066620}},
Article-Number = {{066620}},
ISSN = {{1063-651X}},
Unique-ID = {{ISI:000226299200119}},
}



@article{ YangKaup2000,
Author = {Yang, JK and Kaup, DJ},
Title = {{Stability and evolution of solitary waves in perturbed generalized
   nonlinear Schrodinger equations}},
Journal = {{SIAM JOURNAL ON APPLIED MATHEMATICS}},
Year = {{2000}},
Volume = {{60}},
Number = {{3}},
Pages = {{967-989}},
Month = {{MAR 21}},
ISSN = {{0036-1399}},
Unique-ID = {{ISI:000086058700010}},
}



@article{ Nixon2009,
Author = {Ablowitz, Mark J. and Horikis, Theodoros P. and Nixon, Sean D. and Zhu,
   Yi},
Title = {{Asymptotic Analysis of Pulse Dynamics in Mode-Locked Lasers}},
Journal = {{STUDIES IN APPLIED MATHEMATICS}},
Year = {{2009}},
Volume = {{122}},
Number = {{4, Sp. Iss. 2}},
Pages = {{411-425}},
Month = {{MAY}},
ISSN = {{0022-2526}},
Unique-ID = {{ISI:000266557000005}},
}


@article{Yang2001,
Author = {Yang, JK},
Title = {{Interactions of vector solitons}},
Journal = {{PHYSICAL REVIEW E}},
Year = {{2001}},
Volume = {{64}},
Number = {{2, Part 2}},
Month = {{AUG}},
Article-Number = {{026607}},
ISSN = {{1063-651X}},
Unique-ID = {{ISI:000170493100093}},
}


@article{ Burtsev97,
Author = {Burtsev, S and Camassa, R},
Title = {{Nonadiabatic dynamics of dark solitons}},
Journal = {{JOURNAL OF THE OPTICAL SOCIETY OF AMERICA B-OPTICAL PHYSICS}},
Year = {{1997}},
Volume = {{14}},
Number = {{7}},
Pages = {{1782-1787}},
Month = {{JUL}},
ISSN = {{0740-3224}},
Unique-ID = {{ISI:A1997XL99900034}},
}



